Human Delegation Behavior in Human-AI Collaboration: The Effect of Contextual Information

The integration of artificial intelligence (AI) into human decision-making processes at the workplace presents both opportunities and challenges. One promising approach to leverage existing complementary capabilities is allowing humans to delegate individual instances of decision tasks to AI. However, enabling humans to delegate instances effectively requires them to assess several factors. One key factor is the analysis of both their own capabilities and those of the AI in the context of the given task. In this work, we conduct a behavioral study to explore the effects of providing contextual information to support this delegation decision. Specifically, we investigate how contextual information about the AI and the task domain influence humans' delegation decisions to an AI and their impact on the human-AI team performance. Our findings reveal that access to contextual information significantly improves human-AI team performance in delegation settings. Finally, we show that the delegation behavior changes with the different types of contextual information. Overall, this research advances the understanding of computer-supported, collaborative work and provides actionable insights for designing more effective collaborative systems.

==> old.tex <==
\section{Introduction}
\label{sec: Introduction}

The growth of artificial intelligence (AI) has fundamentally reshaped domains ranging from healthcare over manufacturing to finance \cite{Raees2023, Gmeiner2023, Liu20222, yu_artificial_2018}. In many fields, AI can not just assist humans in their decision-making (e.g., by providing relevant inputs), but even solve particular decision task instances independently. Still, the collaboration with human decision-makers is typically required---and poses a considerable design challenge for computer-supported and cooperative work (CSCW) systems: On the one hand, it is economically meaningful to exploit complementary capabilities of humans and AI \cite{hemmer2022forming, hemmer2022effect}; on the other, regulatory frameworks often require human-in-the-loop concepts \citep{zanzotto2019human} to retain human oversight \citep{european_commision_european_2023}.

Despite the remarkable capabilities of AI in specialized tasks such as image recognition and natural language processing, its integration into human workflows remains a complex challenge \cite{Cabitza2023}. In particular, the effectiveness of AI is fundamentally linked to how people perceive, understand, and ultimately use these systems \cite{LOGG201990, Cabitza2023, SUTTON2023100626, chong2022human}. Delegation serves as one of the primary coordination concepts in human-AI collaboration \cite{fugener2022cognitive, taudien2022calibrating, hemmer2023human, taudien2022effect}: CSCW systems enable humans to identify (and delegate) those task instances to an AI for which the AI is capable of more effectively or efficiently performing the task, and to conduct remaining task instances themselves \cite{fugener2022cognitive}. The effectiveness of this delegation---as the allocation of instances to humans or AI---is a critical challenge for integrating AI into workplace systems.

Understanding the factors that guide humans in passing instances to an AI is increasingly relevant for appropriately designing CSCW systems for human-AI collaboration. Recent research suggests that two factors are essential in this context: the perceived difficulty of the instance \cite{spitzer2023perception} and the human perception of efficacy \cite{hemmer2023human, pinski2023ai}---both an individual's belief in their ability to successfully execute tasks (self-efficacy) and the ability attributed to the AI (AI efficacy). Existing works suggest that instances perceived as more difficult by the human are more frequently delegated to the AI \cite{pinski2023ai, steffel2018delegating}. However, this decision does not necessarily align with the objective difficulty of the instance or the AI’s actual capabilities. Likewise, the human’s perceived self-efficacy for individual instances can have significant implications for delegation decisions \cite{fugener2022cognitive, hemmer2023human}:  An increased sense of self-efficacy may reduce the preference to delegate tasks to an AI, even if it is more capable \cite{taudien2022calibrating, fugener2022cognitive}. Conversely, low self-efficacy could result in overdelegation, bypassing opportunities to apply human expertise and judgment \cite{Cabitza2023}. Similarly, the perception of the AI's efficacy plays a critical role \cite{pinski2023ai}. Discrepancies in the perceived capabilities of AI, whether over- or underestimation, may cause ineffective delegation decisions. Given the influence of perceived difficulty and efficacy on delegation behaviors, examining factors that shape these human perceptions is imperative. Among these factors, previous works show that the role of contextual information is paramount in such CSCW settings \citep{kawakami2022improving, holstein2023toward}. Having access to information about the AI or task domain can impact the delegation decisions. Such information may support the human delegator in framing individual instances within a larger context, thereby shaping their perceptions. For example, information about the outcomes associated with particular attributes may reshape the perception of the instance's difficulty, while information about the AI's capabilities may recalibrate perceptions of the AI efficacy. 


The role of this information, particularly with regard to the AI's abilities \cite{cabrera2023improving, bansal2019beyond} and the distribution of the data involved, plays a central role in human-AI collaboration scenarios \cite{pinski2023ai, pinski2023ailiteracy}. An often overlooked nuance is that humans and AI typically begin with different preconditions: Due to its training data, the AI has a specific understanding of the data distribution that humans may not commonly possess \cite{ethayarajh2022understanding}. Conversely, humans may leverage supplemental information or preexisting domain knowledge in their decision-making that is not accessible to the AI \cite{holstein2023toward, hemmer2022effect}. This asymmetry in prior domain knowledge may skew perceptions of difficulty \cite{taudien2022effect}, self- and AI efficacy \cite{hemmer2023human, pinski2023ai} and ultimately hamper effective delegation within CSCW settings. Previous studies have not accounted for this, though, as they often assume that participants do possess a strong understanding of the domain \cite{taudien2022calibrating} and, thus, of the corresponding data distribution---an assumption that does not hold in many real-world applications and workplaces, for example, when onboarding new employees. Other studies have claimed that more information does not necessarily lead to better performance and may even worsen results \cite{dietzmann2022artificial, Eppler2004}. A potential explanation for these findings may be cognitive overload when the amount of incoming information exceeds an individual’s processing capacity. This may cause humans to overlook or misinterpret relevant information \cite{sweller1994cognitive}. Therefore, there is a trade-off to be made in supporting delegation through contextual information to the human delegator.: On the one hand, providing additional context can help bridge the knowledge gap between humans and AI, which can aid in making better-informed delegation decisions \cite{pinski2023ai}. On the other hand, an excessive amount of information can be overwhelming and counterproductive, especially if it is not well organized or presented \cite{abdul2020cogam}. 

Therefore, we explore whether and how the provision of contextual information---about the AI’s performance and the underlying data---impacts the human-AI team performance. We use the term contextual information to describe different types of information on a) the data distribution for specific features of the dataset or b) on the AI’s performance on subgroups of the dataset. More specifically, we investigate whether providing humans with different kinds of information affects their delegation behavior, i.e., their allocation decisions and the resulting human-AI team performance. We conduct a behavioral study in which subjects can assign instances to an AI based on varying contextual information. Specifically, we pursue the following research questions:

\begin{req}[labelindent=1em, labelwidth=0em, label=\textbf{RQ\arabic*}:, ref=\arabic*]
    \item How does the provision of varying types of contextual information impact human-AI team performance in human delegation? \label{rq1} 
    \item What factors mediate the impact of contextual information on the delegation decisions within human-AI teams? \label{rq2}
    \item How do varying types of contextual information, humans’ perceived efficacy, humans’ perceived difficulty influence the delegation behavior?
    \label{rq3}
\end{req}
RQ1: How does the provision of varying types of contextual information impact human-AI team performance in human delegation?
RQ2: What factors mediate the impact of contextual information on the delegation decisions within human-AI teams?
RQ3: How do humans’ perceived efficacy and humans’ perceived difficulty influence the delegation behavior?

To address our research questions, we conduct a between-subjects study (n=240) with four treatments, each receiving different forms of contextual information. For an income prediction task, we measure the impact of these contextual information types on delegation behavior and human-AI collaboration outcomes. To this end, we adopt established metrics from previous research that asses the perceived instance difficulty \cite{spitzer2023perception}, self-efficacy \cite{hemmer2023human}, and the AI efficacy \cite{pinski2023ai}.

The contribution of our work is threefold: First, we show that providing contextual information based on either data distribution or AI performance does not significantly increase the human-AI team performance. Instead, humans need both types of contextual information to increase the human-AI team performance. Second, we reveal underlying human factors that impact the human-AI team performance in delegation settings. When humans have access to both types of contextual information, their perception of the AI efficacy and instance difficulty mediate its impact on the human-AI team performance. Finally, we shed light on how the assessed human factors influence delegation behavior.

Our findings offer valuable insights for future research to build upon our results and advance the understanding of effective human-AI collaborative systems. Likewise, our results reveal guidance for practioners to customize human-AI systems to individuals’ requirements and create more efficient collaborative systems in CSCW settings.

The remainder of this work is structured as follows: First, we outline related literature on human-AI delegation (\Cref{sec: Related Work},) before describing our theoretical development (\Cref{theoretical_section}) and methodology for our empirical study (\Cref{methodology}). Then, we present the results of our work (\Cref{results_section}). After that, we reveal the implications and limitations of our study (\Cref{sec: Limitations}) and conclude our work (\Cref{conclusion_section}).
